Reconstruction Error-based Anomaly Detection with Few Outlying Examples

Reconstruction error-based neural architectures constitute a classical deep learning approach to anomaly detection which has shown great performances. It consists in training an Autoencoder to reconstruct a set of examples deemed to represent the normality and then to point out as anomalies those data that show a sufficiently large reconstruction error. Unfortunately, these architectures often become able to well reconstruct also the anomalies in the data. This phenomenon is more evident when there are anomalies in the training set. In particular when these anomalies are labeled, a setting called semi-supervised, the best way to train Autoencoders is to ignore anomalies and minimize the reconstruction error on normal data. The goal of this work is to investigate approaches to allow reconstruction error-based architectures to instruct the model to put known anomalies outside of the domain description of the normal data. Specifically, our strategy exploits a limited number of anomalous examples to increase the contrast between the reconstruction error associated with normal examples and those associated with both known and unknown anomalies, thus enhancing anomaly detection performances. The experiments show that this new procedure achieves better performances than the standard Autoencoder approach and the main deep learning techniques for semi-supervised anomaly detection.

==> prel_meth.tex <==
%\section{Preliminaries}
%\label{sec:prel}
Specifically, an \textit{Autoencoder} (AE) is a special type of neural network whose output level is aimed to be identical to the input level
and is composed by two main components:
\begin{itemize}
    \item an \emph{encoder} $f$ that compresses the input space into a \emph{latent space}, whose dimension is lower than the input one;
    \item a \emph{decoder} $g$ that reconstructs the input starting from its latent representation.
\end{itemize}
%
In the following, $z=f(\mathbf{x})$ denotes the latent representation of the input data $\mathbf{x}$ and
$\hat{\mathbf{x}} = g(z) = g(f(\mathbf{x}))$ denotes its reconstruction.

Since the aim of an AE is to reconstruct in output the data $\mathbf{x}$ received in input, the loss of the network can be computed as the mean squared error between $\mathbf{x}$ and $\hat{\mathbf{x}}$:

\begin{equation}
    \mathcal{L}(\mathbf{x})=\left|\left|\mathbf{x}-\hat{\mathbf{x}}\right|\right|_2^2.
        \label{eq:base-loss}
\end{equation}

In the unsupervised scenario, \textit{Autoencoder-based anomaly detection} consists in training an Autoencoder
to reconstruct a set of data and then to detect as anomalies
those samples showing largest \emph{reconstruction error}, which is defined as the value assumed by Equation \eqref{eq:base-loss} after the training phase and plays the role of anomaly score.
%
%
This approach is justified by the observation that, since the reconstruction process includes a dimensionality reduction step (\textit{encoding}) followed by a step mapping back representations in the latent space to examples in the original space (\textit{decoding}), regularities should be better compressed and, hopefully, better reconstructed.

Unfortunately, deep non-linear architectures are able to perform high dimensionality reduction while keeping reconstruction error low and often they generalize so well that they can also
well reconstruct anomalies.
This phenomenon happens also in one-class anomaly detection setting.
%when the AE is trained only with object belonging to the normal class, but it is much more evident in supervised and unsupervised settings where the training set contains also anomalies (labelled or unlabelled).

